FastCSP: Accelerated Molecular Crystal Structure Prediction with Universal Model for Atoms

Molecular crystal structure prediction (CSP) is essential for applications in pharmaceuticals and organic electronics. However, CSP remains challenging and computationally intensive due to the need to explore a large search space with sub-kJ/mol accuracy to distinguish between competing polymorphs. While dispersion-inclusive density functional theory (DFT) offers the necessary precision, its computational cost is impractical for a large number of putative structures. Here, we present FastCSP, an open-source, end-to-end CSP workflow driven entirely by a single pretrained universal machine learning interatomic potential (MLIP), the Universal Model for Atoms (UMA), without any system-specific fine-tuning or DFT calculations. FastCSP integrates conformer generation, random structure generation via Genarris 3, geometry optimization, free energy evaluation, and conformer energy corrections, all powered by UMA. Benchmarked on 28 semi-rigid and 10 flexible molecules spanning 74 experimental polymorphs, FastCSP reliably recovers all known structures, ranking them within 9 kJ/mol of the global minimum. UMA reproduces dispersion-inclusive DFT results with high fidelity across chemically diverse compounds. Conformer corrections are particularly beneficial for flexible compounds with conformational polymorphism, such as ROY. UMA's accuracy, transferability, and computational cost thus eliminate the need for classical force fields in early-stage screening and DFT-based re-ranking in CSP workflows. The open-source release of the entire FastCSP workflow lowers the barrier to accessing CSP, enabling both pharmaceutical-grade and high-throughput polymorph screening within practical computational reach.

==> assets/comments.tex <==
%UMA accurately reproduced the PBE-D3 Gibbs free energy, with a mean absolute error of only 0.29 kJ/mol at 300 K. UMA also achieved excellent agreement with experimental entropy data~\cite{glycine_exp_data, glycine_rank3}, showing deviations of just 4.53 J/mol/K, 4.29 J/mol/K, and 4.62 J/mol/K for $\alpha$, $\beta$ and $\gamma$, respectively, at 300 K.


The UMA results are in close agreement with PBE-D3 and in good agreement with experiment for all three forms of glycine. At 300 K, the specific heat values obtained with both UMA and PBE-D3 are slightly underestimated compared to experiment. 
%with deviations of 9.15 J/mol/K, 7.27 J/mol/K, and 6.10 J/mol/K, respectively,


%\clearpage
%\newpage
%\bibliographystyle{assets/plainnat}
%\bibliographystyle{unsrtnat}
%\bibliographystyle{achemso}
%\mciteErrorOnUnknownfalse


crystal overlays
    % & & \textbf{CILJIQ$\bigtria$} & 0.24  &   \\
    % & & \textbf{CILJIQ01$\star$} & - & - & - & - & - & - & &  \\
% \multicolumn{5}{c}%
% {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\



 % \begin{figure}[h!tbp]
 %     \centering
 %     \includegraphics[width=0.5\textwidth]{figs/rmsd_corr.pdf}
 %     \caption{Deviation of input conformers and matched crystals in FastCSP from the experimental conformers and crystals, respectively. Shown are the RMSD between the FHI-aims relaxed conformer and the experimental conformer, and RMSD$_{30}$ between the UMA predicted match and the experimental structure.}
 %     \label{fig:rmsd_corr}
 % \end{figure}


 Schrodinger rel energies table
     % & & $\delta$ & 2.72 & 11 & &  &  &\\
    % & & $\varepsilon$ & 1.59 & 5 & - & - & - & -\\


 %($\sim 12\%$ of the structures were not converged)

dataset
          % & & GLYCIN50 & 2 & 7 ($Pn$) & $\delta$ [2.7-7.8 GPa]~\cite{glycine_p1} & 293 K \\

                  % \multirow{2}{*}{22} & \multirow{2}{*}{1,2-Cyclohexanedicarboximide} & \multirow{2}{*}{FastCSP Target CHDI} & IHEPUG & 8 & 92 ($P4_12_12$) & - & 293 K \\
         % & & & IHEPUG02 & 4 & 19 ($P2_12_12_1$) & - & 203 K \\

                  % & & & NICOAM07 & 2 & 4 ($P2_1$) & $\varepsilon$ & 100 K \\ different conformers
